Catalysis by Dark States in Vibropolaritonic Chemistry

Collective strong coupling between a disordered ensemble of $N$ localized molecular vibrations and a resonant optical cavity mode gives rise to 2 polariton and $N-1\gg2$ dark modes. Thus, experimental changes in thermally-activated reaction kinetics due to polariton formation appear entropically unlikely and remain a puzzle. Here we show that the overlooked dark modes, while parked at the same energy as bare molecular vibrations, are robustly delocalized across $\sim$2-3 molecules, yielding enhanced channels of vibrational cooling, concomitantly catalyzing a chemical reaction. As an illustration, we theoretically show a $\approx$50\% increase in an electron transfer rate due to enhanced product stabilization. The reported effects can arise when the homogeneous linewidths of the dark modes are smaller than their energy spacings.

==> auxSI.tex <==


